A systematic analysis of star cluster disruption by tidal shocks -- II. Predicting star cluster dissolution rates from a time-series analysis of their tidal histories

Most of the dynamical mass loss from star clusters is thought to be caused by the time-variability of the tidal field (``tidal shocks''). Systematic studies of tidal shocks have been hampered by the fact that each tidal history is unique, implying both a reproducibility and a generalisation problem. Here we address these issues by investigating how star cluster evolution depends on the statistical properties of its tidal history. We run a large suite of direct N-body simulations of clusters with tidal histories generated from power spectra of a given slope and with different normalisations, which determine the time-scales and amplitudes of the shocks, respectively. At fixed normalisation (i.e. the same median tidal field strength), the dissolution time-scale is nearly independent of the power spectrum slope. However, the dispersion in dissolution time-scales, obtained by repeating simulations for different realisations of statistically identical tidal histories, increases with the power spectrum slope. This result means that clusters experiencing high-frequency shocks have more similar mass loss histories than clusters experiencing low-frequency shocks. The density-mass relationship of the simulated clusters follows a power-law with slope between 1.08 and 1.45, except for the lowest normalisations (for which clusters effectively evolve in a static tidal field). Our findings suggest that star cluster evolution can be described statistically from a time-series analysis of its tidal history, which is an important simplification for describing the evolution of the star cluster population during galaxy formation and evolution.

==> referee_feedback.tex <==
We would like to thank the referee for their constructive report. Their comments have certainly improved the manuscript. The comments have been copied below with our responses marked with a -->. Changes to the manuscript are marked in bold. 

Referee Comments:

1.- As stated in the text, T_xx is larger or equal to zero, with all other components of the tidal tensor set to zero; and I notice that it is the same for Paper I. However, this implies that the trace of the tidal tensor is always positive (or zero), which is not a physical scenario. Hence, I think this should be addressed in the text, including a justification of why the authors decided to use tidal tensors that do not correspond to a positive mass density.

--> We have added text to Section 2 that justify how we setup or tidal histories. Similar to Paper I, we are looking to do a systematic exploration how cluster evolution is affected by tidal shocks. Hence we were motivated to begin with simplified, 1-Dimensional tensors to see how strongly cluster evolution is correlated with the evolution of this single parameter. This simplified approach allows us to minimize the complexity of the experimental setup and more easily interpret the results. We also remind the readers in the conclusion that our tensors imply a perturber with negative mass density.

IN THE PAPER (BUT WON'T BE INCLUDED IN THE REPORT):

Section 2:

\textbf{While the strength and time-variation in our tidal histories are comparable to the maximum eigenvalues of tidal histories extracted from EMP-Pathfinder, it remains important to remember that our generated histories are not physical in that they don't represent interactions between a cluster and substructure. Our tidal tensors are all one dimensional with only $T_{xx}$ being assigned positive values based on our method for generating tidal histories from a power spectrum. Hence the shocks are extensive and only occur along the x-axis, with the positive trace of the tidal tensor implying a negative mass density. Similar to \citetalias{Webb2019a}, using such idealised tensors allow for a systematic study of how star clusters are affected by tidal shocks since the number of free parameters in the experimental setup have been minimized. By first establishing a relationship between cluster evolution and the global properties of these simplified tidal histories, in this case governed by two parameters, we form a basis for expanding this approach to more complex tidal histories.}

Conclusion:

\textbf{As noted in Section \ref{sec:nbody}, our tidal histories imply a perturber with a negative mass density.}

2.- How will these results hold in more realistic setups? For example, in realistic tidal fields that include extensive and compressive modes; or in simulations that include stellar evolution, leading to the presence of black holes, which can be important in the evolution of the density and mass loss of star clusters. I understand that this exploration is beyond the scope of this paper, but the authors could expand the discussion on these extra free parameters. 

--> We now note in the conclusions that the applicability of these results will depend strongly on how well the effects of tidal heating on cluster evolution can be approximated by the time-evolution of a single parameter (i.e. the maximum eigenvalue of the tidal tensor as a function of time). A complete model would then also have to include the effects of stellar evolution and relaxation, which will introduce additional free parameters into the problem.

IN THE PAPER (BUT WON'T BE INCLUDED IN THE REPORT):

\textbf{While the results of our study imply the effects of tidal heating on cluster evolution could be approximated based on a Fourier analysis of its tidal history, it does not take into account other factors known to govern cluster evolution. Stellar evolution is known to strongly affect early cluster evolution and relaxation is capable to affecting the evolution of clusters with longer dissolution times \citep{heggie03}. While tidal shocks are the dominant external mass loss mechanism experience by clusters, these other processes must be explored before developing a complete model for how clusters evolve in a time-dependent tidal field.}


3.- Finally, and related to the previous points, Could it be that the statistical description of star cluster evolution works only because of the simplified tidal tensors used here?

--> This question is difficult to answer without another large suite of simulations, however we have highlight this question in the text added to the conclusion in response to points 1 and 2.

IN THE PAPER (BUT WON'T BE INCLUDED IN THE REPORT):

\textbf{However, it is possible that a statistical description of a star cluster's evolution is only possible with simplified tidal histories such as ours.}

Minor points:

There is a typo in Fig. 3, the label should read S10 instead of S03.
--> Typo fixed
